X-ray Luminosity Functions of Normal Galaxies in the GOODS

We present soft (0.5-2 keV) X-ray luminosity functions (XLFs) in the Great Observatories Origins Deep Survey (GOODS) fields, derived for galaxies at z~0.25 and 0.75. SED fitting was used to estimate photometric redshifts and separate galaxy types, resulting in a sample of 40 early-type galaxies and 46 late-type galaxies. We estimate k-corrections for both the X-ray/optical and X-ray/NIR flux ratios, which facilitates the separation of AGN from the normal/starburst galaxies. We fit the XLFs with a power-law model using both traditional and Markov-Chain Monte Carlo (MCMC) procedures. The XLFs differ between z<0.5 and z>0.5, at >99% significance levels for early-type, late-type and all (early and late-type) galaxies.We also fit Schechter and log-normal models to the XLFs, fitting the low and high redshift XLFs for a given sample simultaneously assuming only pure luminosity evolution. In the case of log-normal fits, the results of MCMC fitting of the local FIR luminosity function were used as priors for the faint and bright-end slopes (similar to ``fixing'' these parameters at the FIR values except here the FIR uncertainty is included). The best-fit values of the change in log L* with redshift were dlogL* = 0.23 +/- 0.16 dex (for early-type galaxies) and 0.34 +/- 0.12 dex (for late-type galaxies), corresponding to (1+z)^1.6 and (1+z)^2.3. These results were insensitive to whether the Schechter or log-normal function was adopted.

==> tab7.tex <==
48& 1.01& 4& 0.27& agn2& 38.53& 0.90& 42.16 & -1.97 & -2.99 & early &\\
55& 0.64& 1& 0.12& & \ldots& \ldots& 41.30 & -2.78 & -3.02 & late &\\
56& 0.13& 4& 0.20& gal& 14.16& 0.51& 39.94 & -2.72 & -2.30 & late & & 0.08$^{a\dagger}$\\
57& 0.38& 2& 0.15& gal& 12.78& 1.36& 40.87 & -3.21 & -3.33 & late & E (0.38) & 0.33$^{a\dagger}$\\
60& 0.42& 4& 0.05& & \ldots& \ldots& 40.54 & -2.42 & -2.52 & early &\\
62& 0.22& 4& 0.03& gal& 18.12& 1.21& 39.58 & -4.56 & -4.44 & early & A (0.09)\\
67& 0.64& 1& 0.14& gal& 8.68& 0.98& 41.39 & -2.87 & -3.30 & late & & 0.64$^{a}$\\
72& 0.94& 1& 0.11& & \ldots& \ldots& 41.68 & -2.36 & -2.97 & late &\\
78& 0.75& 1& 0.18& agn2& 1.39& 1.14& 41.66 & -1.72 & -2.24 & early & & 0.75$^{a}$\\
81& 0.38& 4& 0.10& gal& 10.92& 0.84& 40.70 & -3.12 & -3.28 & early &\\
82& 0.68& 1& 0.14& & \ldots& \ldots& 41.44 & -2.58 & -2.87 & early &\\
87& 0.14& 1& 0.12& gal& 20.57& 1.31& 39.76 & -3.39 & -3.20 & early & A (0.14)\\
90& 1.14& 1& 0.16& agn2& 13.13& 0.84& 42.06 & -2.09 & -2.88 & late &\\
93& 0.28& 1& 5.08& agn2& 1.80& 2.12& 42.08 & -1.70 & -1.75 & late &\\
101& 0.45& 1& 0.08& gal& 12.60& 1.19& 40.81 & -3.08 & -3.30 & early & A (0.45) & 0.45$^{a}$\\
103& 0.97& 2& 0.28& agn2& 1.51& 0.66& 42.13 & -2.05 & -2.62 & late & & 0.81$^{a\dagger}$\\
105& 0.33& 4& 0.03& gal& 14.66& 0.96& 40.03 & -3.31 & -3.41 & early &\\
110& 1.01& 4& 0.34& agn2& 0.89& 1.05& 42.26 & -1.98 & -2.54 & early &\\
111& 0.52& 1& 0.04& gal& 13.33& 1.15& 40.64 & -3.17 & -3.57 & late & E (0.52) & 0.52$^{a}$\\
113& 0.84& 2& 1.59& agn1& 4.98& 1.93& 42.74 & -1.29 & -1.90 & late & & 0.84$^{a}$\\
114& 0.53& 1& 0.04& gal& 17.54& 0.65& 40.63 & -3.22 & -3.53 & early &\\
115& 0.68& 1& 4.67& agn1& 5.48& 1.43& 42.98 & -1.21 & -1.38 & late & & 0.68$^{a}$\\
119& 0.47& 1& 0.08& gal& 12.31& 1.14& 40.83 & -3.11 & -3.35 & early & E (0.47) & 0.47$^{a}$\\
120& 0.69& 1& 0.09& gal& 7.17& 0.51& 41.27 & -2.78 & -2.75 & ir &\\
126& 0.77& 4& 0.03& gal& 10.68& 0.93& 40.90 & -3.01 & -3.60 & late & & 0.84$^{a}$\\
132& 0.64& 1& 0.07& gal& 11.36& 0.67& 41.06 & -3.01 & -3.26 & late & E (0.65) & 0.64$^{a}$\\
136& 0.47& 1& 0.05& gal& 13.55& 1.16& 40.65 & -3.20 & -3.37 & early & A (0.47) & 0.47$^{a}$\\
138& 0.48& 1& 0.07& gal& 10.81& 0.80& 40.80 & -2.92 & -3.05 & late & E (0.48) & 0.48$^{a}$\\
139& 0.93& 4& 0.76& agn1& 2.87& 0.75& 42.52 & -1.60 & -2.20 & late & & 1.01$^{a}$\\
142& 0.75& 1& 0.29& agn2& 7.05& 0.97& 41.87 & -2.02 & -2.60 & early &\\
150& 0.63& 4& 0.13& agn2& 23.99& 1.38& 41.35 & -1.85 & -2.26 & early &\\
158& 1.01& 2& 0.17& agn2& 20.44& 0.49& 41.96 & -2.16 & -3.33 & early &\\
160& 0.82& 4& 0.12& & \ldots& \ldots& 41.57 & -2.73 & -2.91 & late &\\
166& 0.46& 1& 0.04& & \ldots& \ldots& 40.50 & -2.78 & -2.63 & late & & 0.46$^{a}$\\
169& 0.31& 4& 0.10& gal& 13.84& 1.10& 40.48 & -3.08 & -3.09 & late & A (0.84)\\
170& 0.63& 4& 0.20& agn2& 11.44& 0.77& 41.53 & -2.13 & -2.62 & early &\\
177& 1.02& 1& 0.25& agn2& 2.73& 0.66& 42.14 & -2.07 & -2.99 & late & & 1.01$^{a}$\\
180& 0.46& 1& 0.23& gal& 9.37& 1.05& 41.25 & -2.97 & -3.35 & early & & 0.46$^{a}$\\
187& 0.94& 4& 0.04& gal& 14.53& 0.49& 41.23 & -2.80 & -3.68 & late &\\
188& 1.15& 5& 0.07& agn2& 4.05& 0.88& 41.71 & -1.93 & -2.47 & late &\\
189& 0.41& 1& 0.17& & \ldots& \ldots& 41.01 & -2.57 & -2.71 & early &\\
194& 0.56& 1& 1.62& agn1& 6.01& 2.94& 42.30 & -1.19 & -1.41 & late & & 0.56$^{a}$\\
197& 0.08& 1& 0.05& gal& 28.79& 0.90& 38.90 & -3.81 & -3.43 & late & E (0.08) & 0.08$^{a}$\\
200& 0.97& 1& 0.04& & \ldots& \ldots& 41.31 & -2.72 & -3.18 & late &\\
203& 1.14& 2& 0.03& gal& 10.14& 0.98& 41.27 & -3.02 & -3.96 & late &\\
209& 0.51& 2& 0.23& & \ldots& \ldots& 41.36 & -2.13 & -2.47 & late & & 0.51$^{a}$\\
210& 0.70& 4& 0.09& gal& 8.43& 0.87& 41.30 & -2.71 & -3.30 & early &\\
211& 0.76& 4& 0.06& gal& 8.76& 0.51& 41.23 & -2.82 & -3.10 & late & & 0.85$^{a}$\\
212& 0.94& 1& 0.13& & \ldots& \ldots& 41.77 & -2.28 & -2.76 & early &\\
214& 1.04& 4& 0.03& gal& 8.63& 0.75& 41.27 & -2.93 & -3.63 & early &\\
215& 1.01& 2& 0.03& & \ldots& \ldots& 41.17 & -2.22 & -3.63 & late &\\
217& 0.54& 4& 0.04& gal& 24.31& 0.79& 40.63 & -3.38 & -3.97 & early &\\
218& 0.09& 1& 0.10& gal& 21.17& 0.65& 39.31 & -3.05 & -2.65 & late & E (0.09)\\
219& 0.70& 4& 0.03& gal& 10.65& 0.85& 40.76 & -3.02 & -3.64 & early &\\
222& 0.77& 4& 0.59& agn2& 3.17& 1.29& 42.21 & -1.88 & -2.60 & early & & 0.86$^{a}$\\
227& 0.52& 4& 0.04& gal& 13.17& 1.03& 40.57 & -3.14 & -3.34 & late & E (0.56) & 0.56$^{a}$\\
230& 1.01& 1& 0.08& gal& 9.67& 1.11& 41.62 & -2.99 & -3.80 & early & & 1.01$^{a}$\\
234& 0.45& 1& 0.09& gal& 10.56& 0.84& 40.85 & -2.89 & -2.97 & late & & 0.45$^{a}$\\
244& 0.97& 1& 0.05& gal& 9.90& 0.91& 41.36 & -3.06 & -3.67 & late & & 0.97$^{a}$\\
245& 0.32& 1& 0.02& gal& 15.27& 0.81& 39.90 & -3.32 & -3.09 & late & E (0.32) & 0.32$^{a}$\\
249& 0.47& 2& 0.24& & \ldots& \ldots& 41.30 & -2.53 & -2.71 & early &\\
251& 0.14& 1& 0.07& gal& 22.92& 1.31& 39.59 & -3.59 & -3.24 & late & E (0.14) & 0.14$^{a}$\\
256& 0.60& 1& 0.09& & \ldots& \ldots& 41.10 & -2.65 & -2.72 & late &\\
257& 0.09& 1& 0.04& gal& 30.11& 1.08& 38.92 & -4.09 & -3.93 & early & A (0.09)\\
258& 0.75& 1& 0.04& gal& 9.97& 0.79& 40.96 & -2.83 & -3.34 & late & & 0.75$^{a}$\\
260& 0.47& 1& 0.06& gal& 10.82& 0.86& 40.71 & -2.69 & -3.13 & late & & 0.47$^{b}$\\
262& 0.87& 4& 0.67& agn1& 4.47& 1.93& 42.39 & -1.31 & -1.91 & early & & 0.81$^{b\dagger}$\\
264& 0.32& 1& 0.05& & \ldots& \ldots& 40.25 & -2.54 & -2.29 & late & & 0.32$^{b}$\\
265& 0.41& 1& 0.09& gal& 12.74& 1.30& 40.74 & -3.03 & -3.35 & early & C (0.41) & 0.41$^{b}$\\
266& 1.08& 4& 0.04& & \ldots& \ldots& 41.38 & -2.36 & -3.67 & early &\\
269& 0.36& 2& 0.05& & \ldots& \ldots& 40.36 & -2.56 & -2.42 & late & & 0.36$^{b}$\\
274& 0.32& 1& 0.24& gal& 10.66& 1.13& 40.91 & -3.01 & -3.13 & early & A (0.32)\\
278& 1.02& 2& 0.03& & \ldots& \ldots& 41.24 & -2.49 & -3.16 & late &\\
279& 0.89& 2& 0.03& & \ldots& \ldots& 41.07 & -2.46 & -2.92 & ir &\\
280& 0.96& 4& 0.04& & \ldots& \ldots& 41.25 & -2.23 & -2.90 & early &\\
282& 0.20& 2& 0.06& gal& 18.94& 1.10& 39.87 & -3.42 & -3.42 & late & E (0.20) & 0.08$^{b\dagger}$\\
286& 0.95& 1& 0.41& agn2& 0.71& 1.16& 42.28 & -1.92 & -2.61 & early & & 0.95$^{b}$\\
288& 0.71& 4& 0.11& gal& 8.51& 0.88& 41.38 & -2.61 & -3.54 & early & & 0.79$^{b}$\\
291& 0.52& 1& 0.04& gal& 14.27& 1.20& 40.60 & -3.35 & -3.62 & early &\\
292& 0.50& 2& 0.02& & \ldots& \ldots& 40.34 & -2.27 & -2.46 & ir &\\
294& 0.47& 2& 0.31& agn2& 1.29& 1.50& 41.42 & -1.50 & -1.93 & late & & 0.47$^{b}$\\
295& 0.85& 1& 0.06& & \ldots& \ldots& 41.31 & -2.36 & -2.68 & late &\\
296& 0.66& 1& 0.07& gal& 11.67& 0.55& 41.12 & -2.89 & -3.30 & early &\\
300& 0.14& 2& 0.07& gal& 25.94& 1.48& 39.54 & -3.91 & -3.75 & late & E (0.14) & 0.14$^{b}$\\
304& 0.68& 1& 3.22& agn1& 5.87& 2.60& 42.81 & -1.30 & -1.75 & late &\\
305& 0.30& 1& 0.05& gal& 17.69& 1.30& 40.15 & -3.43 & -3.47 & late & E (0.30) & 0.30$^{b}$\\
309& 1.14& 2& 0.68& agn1& 4.25& 1.77& 42.70 & -1.37 & -2.28 & late & & 1.14$^{b}$\\
310& 0.76& 1& 0.03& gal& 11.44& 1.02& 40.91 & -3.05 & -3.64 & late & & 0.76$^{b}$\\
311& 0.91& 1& 0.05& gal& 7.15& 0.49& 41.33 & -2.56 & -3.18 & late & & 0.91$^{b}$\\
313& 0.80& 1& 0.07& gal& 9.70& 0.88& 41.30 & -3.08 & -3.71 & early &\\
320& 0.14& 1& 0.05& gal& 23.11& 1.04& 39.40 & -3.53 & -3.25 & late & E (0.14) & 0.14$^{b}$\\
323& 0.51& 1& 6.48& agn2& 11.69& 3.65& 42.82 & -1.37 & -1.55 & late &\\
326& 0.36& 2& 0.05& & \ldots& \ldots& 40.29 & -3.00 & -3.24 & late &\\
332& 0.56& 1& 0.04& gal& 16.42& 0.71& 40.70 & -3.13 & -3.54 & late &\\
333& 0.38& 1& 0.86& agn2& 0.95& 0.97& 41.62 & -1.96 & -2.01 & late & & 0.38$^{b}$\\
337& 0.90& 1& 0.03& gal& 12.22& 0.90& 41.04 & -3.31 & -3.79 & late &\\
339& 0.25& 1& 0.05& gal& 22.38& 1.14& 39.95 & -3.82 & -3.84 & late & E (0.25) & 0.25$^{b}$\\
344& 0.09& 4& 15.70& agn1& 4.26& 0.99& 41.50 & -1.06 & -0.78 & ir &\\
346& 1.02& 2& 0.02& gal& 7.37& 0.69& 40.98 & -2.80 & -3.76 & late & & 1.02$^{b}$\\
349& 1.12& 4& 0.53& agn1& 3.71& 1.23& 42.56 & -1.14 & -2.45 & early & & 1.25$^{b\dagger}$\\
351& 0.94& 1& 0.09& gal& 7.85& 0.50& 41.59 & -2.64 & -3.53 & late & & 0.94$^{b}$\\
352& 0.91& 4& 0.03& gal& 17.62& 0.69& 41.13 & -3.12 & -3.84 & late &\\
353& 0.42& 1& 0.10& gal& 11.41& 1.05& 40.80 & -2.97 & -3.06 & late & C (0.42) & 0.42$^{b}$\\
354& 0.57& 2& 0.09& & \ldots& \ldots& 41.05 & -2.53 & -2.70 & early &\\
367& 0.78& 4& 0.17& agn2& 2.27& 1.19& 41.68 & -1.65 & -2.41 & early &\\
373& 0.48& 1& 0.15& agn2& 22.40& 0.52& 41.11 & -2.35 & -2.68 & early &\\
378& 1.08& 2& 0.04& & \ldots& \ldots& 41.40 & -2.35 & -2.98 & late & & 1.08$^{b}$\\
383& 0.17& 4& 0.05& gal& 25.18& 1.47& 39.63 & -4.05 & -3.88 & early & A (0.11) & 0.11$^{b}$\\
384& 1.02& 2& 0.09& & \ldots& \ldots& 41.70 & -2.30 & -3.39 & early &\\
387& 0.97& 4& 0.08& & \ldots& \ldots& 41.59 & -2.20 & -2.99 & early & & 1.01$^{b\dagger}$\\
389& 0.56& 1& 0.05& & \ldots& \ldots& 40.79 & -2.52 & -3.15 & late &\\
392& 0.40& 4& 0.05& gal& 14.47& 1.13& 40.48 & -3.24 & -3.50 & early & E (0.41) & 0.41$^{b}$\\
401& 0.94& 1& 0.07& gal& 7.52& 0.63& 41.52 & -2.63 & -3.44 & early &\\
404& 0.11& 1& 0.07& gal& 25.62& 1.11& 39.27 & -3.76 & -3.56 & late & A (0.11)\\
405& 0.94& 4& 0.05& & \ldots& \ldots& 41.38 & -2.80 & -3.56 & late &\\
414& 0.80& 1& 0.09& & \ldots& \ldots& 41.45 & -2.46 & -2.91 & early &\\
418& 0.28& 1& 0.09& gal& 17.04& 1.26& 40.34 & -3.50 & -3.47 & late & & 0.28$^{b}$\\
426& 0.16& 2& 0.08& agn2& 12.68& 0.75& 39.75 & -2.17 & -1.80 & ir &\\
428& 0.30& 2& 0.10& gal& 14.84& 1.05& 40.47 & -3.23 & -3.13 & late & E (0.30)\\
433& 1.04& 4& 0.08& gal& 7.72& 0.69& 41.66 & -2.70 & -3.61 & early & & 1.02$^{b}$\\
437& 0.82& 4& 0.85& agn1& 2.18& 0.54& 42.44 & -1.80 & -2.37 & late & & 0.84$^{b}$\\
453& 0.73& 4& 0.38& agn2& 2.17& 0.59& 41.96 & -2.13 & -2.74 & early & & 0.84$^{b}$\\
454& 0.46& 4& 0.39& & \ldots& \ldots& 41.48 & -2.26 & -2.45 & early & & 0.46$^{b}$\\
458& 0.07& 1& 0.31& & \ldots& \ldots& 39.57 & -3.03 & -2.78 & late &   (0.07)\\
462& 0.51& 1& 0.03& & \ldots& \ldots& 40.44 & -3.21 & -3.36 & early &\\
466& 0.44& 1& 0.09& gal& 13.55& 1.16& 40.81 & -3.15 & -3.65 & early &\\
471& 1.17& 2& 0.10& gal& 7.89& 0.64& 41.90 & -2.71 & -3.71 & early &\\
473& 0.31& 1& 24.90& agn1& 7.71& 3.56& 42.88 & -1.12 & -1.25 & late &\\
477& 0.44& 1& 0.10& & \ldots& \ldots& 40.86 & -2.67 & -2.82 & early &\\
478& 0.08& 4& 2.27& agn2& 4.40& 2.84& 40.55 & -1.03 & -0.82 & early &\\
480& 0.46& 1& 0.20& & \ldots& \ldots& 41.19 & -2.28 & -2.77 & early &\\


==> tab8.tex <==
29& 0.57& 1& 0.24& gal& 7.12& 0.81& 41.51 & -3.25 & \ldots & early\\
44& 0.57& 1& 0.60& & \ldots& \ldots& 41.91 & -2.96 & \ldots & early\\
53& 0.67& 1& 0.14& & \ldots& \ldots& 41.43 & -2.57 & -2.95 & early\\
60& 0.54& 1& 0.23& & \ldots& \ldots& 41.44 & -2.53 & \ldots & late\\
73& 0.42& 1& 0.10& gal& 13.41& 1.22& 40.78 & -3.62 & -3.81 & early\\
75& 1.00& 1& 0.08& gal& 6.74& 0.48& 41.61 & -2.81 & -3.45 & late\\
80& 0.58& 1& 0.23& agn2& 6.17& 0.77& 41.49 & -2.21 & -2.38 & early\\
83& 0.68& 1& 0.06& gal& 9.35& 0.76& 41.11 & -3.00 & -3.39 & early\\
84& 1.03& 1& 0.15& & \ldots& \ldots& 41.93 & -2.30 & -3.28 & late\\
88& 0.60& 1& 2.48& agn2& 21.15& 2.29& 42.58 & -1.87 & -2.12 & late\\
94& 0.12& 1& 0.73& agn2& 30.05& 2.26& 40.45 & -1.43 & -1.69 & late\\
103& 0.68& 1& 1.76& agn1& 3.64& 1.47& 42.54 & -1.68 & -2.06 & early\\
106& 0.67& 1& 0.27& agn2& 1.67& 0.50& 41.72 & -1.98 & -2.45 & early\\
113& 0.52& 1& 0.09& & \ldots& \ldots& 40.97 & -2.45 & -2.49 & early\\
115& 0.34& 1& 0.06& gal& 18.63& 1.06& 40.33 & -3.66 & -3.84 & early\\
117& 0.57& 1& 4.50& agn1& 7.26& 3.69& 42.77 & -1.19 & -1.46 & late\\
118& 1.10& 1& 0.55& agn2& 38.53& 1.68& 42.56 & -1.80 & -2.60 & early\\
121& 0.73& 1& 0.28& gal& 6.78& 0.80& 41.84 & -2.97 & -3.38 & early\\
122& 0.18& 1& 0.36& agn2& 5.20& 2.97& 40.52 & -0.91 & -0.98 & ir\\
124& 0.96& 1& 0.08& & \ldots& \ldots& 41.56 & -2.51 & -3.06 & late\\
126& 0.59& 4& 0.33& agn2& 5.84& 2.85& 41.67 & -1.17 & -1.55 & early\\
129& 0.23& 1& 0.22& gal& 14.37& 1.15& 40.54 & -3.23 & -3.19 & early\\
134& 0.60& 1& 0.07& & \ldots& \ldots& 41.00 & -2.64 & -3.13 & early\\
146& 0.73& 1& 0.09& & \ldots& \ldots& 41.33 & -2.44 & -3.26 & early\\
149& 0.13& 1& 0.23& & \ldots& \ldots& 40.02 & -2.73 & -2.50 & late\\
152& 0.25& 1& 0.06& gal& 15.29& 0.90& 40.06 & -3.36 & -3.08 & ir\\
155& 0.53& 1& 1.85& agn1& 3.26& 1.37& 42.32 & -1.82 & -1.88 & early\\
158& 0.36& 1& 0.09& gal& 11.29& 0.73& 40.61 & -2.94 & -2.92 & late\\
159& 1.05& 1& 0.91& agn2& 4.15& 3.43& 42.73 & -1.00 & -2.01 & late\\
161& 0.73& 1& 0.31& & \ldots& \ldots& 41.87 & -3.09 & \ldots & late\\
162& 1.04& 1& 0.08& agn2& 8.43& 0.78& 41.65 & -2.17 & -2.54 & late\\
167& 0.58& 1& 0.09& gal& 11.41& 1.00& 41.06 & -3.28 & -3.51 & early\\
169& 1.02& 4& 0.05& & \ldots& \ldots& 41.43 & -3.65 & \ldots & late\\
171& 1.03& 1& 0.18& agn2& 0.64& 1.56& 42.00 & -1.83 & -1.72 & late\\
176& 0.73& 1& 0.61& agn2& 6.11& 1.71& 42.17 & -1.79 & -2.31 & early\\
179& 0.66& 1& 0.49& agn2& 30.04& 1.77& 41.97 & -1.87 & -2.13 & late\\
181& 0.74& 1& 0.25& & \ldots& \ldots& 41.79 & -2.32 & -2.61 & early\\
182& 0.21& 1& 0.67& gal& 10.83& 1.08& 40.95 & -3.13 & -3.06 & early\\
184& 0.62& 1& 1.32& & \ldots& \ldots& 42.33 & -2.86 & \ldots & early\\
185& 0.18& 4& 0.06& agn2& 11.38& 0.60& 39.74 & -2.33 & -1.98 & ir\\
189& 0.08& 1& 0.81& gal& 21.22& 2.08& 40.06 & -3.60 & -3.42 & late\\
190& 1.02& 1& 0.06& & \ldots& \ldots& 41.48 & -2.09 & -2.70 & late\\
192& 0.08& 1& 0.57& gal& 21.21& 1.53& 39.91 & -3.56 & -3.43 & late\\
193& 0.96& 1& 1.81& agn1& 6.23& 3.07& 42.93 & -1.27 & -1.96 & late\\
196& 0.67& 1& 0.07& & \ldots& \ldots& 41.13 & -2.74 & -2.75 & late\\
203& 1.18& 4& 0.04& gal& 6.08& 0.72& 41.54 & -3.29 & -4.12 & early\\
207& 0.10& 1& 0.18& gal& 27.50& 1.25& 39.69 & -4.09 & -4.02 & early\\
210& 0.83& 1& 0.07& & \ldots& \ldots& 41.38 & -2.18 & -2.71 & early\\
212& 0.67& 1& 0.17& & \ldots& \ldots& 41.53 & -2.52 & -2.80 & early\\
214& 0.84& 1& 1.51& agn1& 5.35& 1.98& 42.71 & -1.22 & -1.63 & late\\
224& 0.55& 1& 0.12& gal& 9.46& 0.88& 41.14 & -2.90 & -3.31 & late\\
225& 0.55& 1& 0.06& gal& 11.56& 1.05& 40.83 & -3.21 & -3.62 & late\\
226& 1.00& 1& 0.12& & \ldots& \ldots& 41.79 & -2.19 & -2.71 & late\\
227& 0.67& 1& 4.01& agn1& 7.49& 2.95& 42.89 & -0.90 & -1.19 & early\\
229& 0.67& 1& 1.86& agn1& 3.40& 1.91& 42.55 & -1.59 & \ldots & late\\
236& 0.46& 1& 0.08& gal& 9.70& 0.59& 40.78 & -2.84 & -2.91 & ir\\
238& 0.24& 1& 0.06& gal& 17.46& 1.25& 40.05 & -3.42 & -3.66 & late\\
244& 0.58& 1& 0.12& & \ldots& \ldots& 41.21 & -2.54 & -2.99 & early\\
247& 0.62& 2& 0.54& agn2& 22.40& 0.76& 41.95 & 0.59 & \ldots & early\\
248& 0.67& 4& 0.03& gal& 10.45& 1.02& 40.83 & -3.35 & -3.74 & early\\
256& 0.74& 1& 3.66& agn1& 9.56& 4.09& 42.96 & -0.55 & -0.88 & ir\\
260& 0.27& 1& 0.51& gal& 7.85& 0.95& 41.08 & -2.68 & -2.82 & early\\
262& 0.42& 1& 0.13& gal& 10.01& 0.71& 40.89 & -2.91 & -3.05 & late\\
263& 1.01& 1& 0.56& agn2& 12.02& 2.67& 42.48 & -1.53 & -1.85 & early\\
265& 0.46& 1& 0.14& gal& 9.69& 0.88& 41.04 & -3.48 & \ldots & late\\
266& 0.44& 1& 0.09& gal& 10.56& 0.81& 40.80 & -2.93 & -3.13 & late\\
267& 0.10& 1& 0.11& & \ldots& \ldots& 39.45 & -2.96 & \ldots & ir\\
269& 0.66& 1& 0.22& & \ldots& \ldots& 41.63 & -3.82 & \ldots & early\\
271& 1.18& 1& 0.12& & \ldots& \ldots& 41.96 & -2.32 & -3.04 & late\\
273& 1.11& 1& 0.09& & \ldots& \ldots& 41.79 & -2.30 & -3.02 & late\\
276& 0.67& 1& 0.15& & \ldots& \ldots& 41.47 & -2.99 & -3.43 & early\\
277& 1.15& 4& 0.78& agn1& 2.04& 1.16& 42.76 & -0.31 & \ldots & late\\
292& 0.37& 1& 0.22& & \ldots& \ldots& 41.01 & -2.70 & -2.42 & ir\\
293& 1.14& 1& 0.18& gal& 8.46& 0.49& 42.13 & -4.43 & -2.47 & early\\
303& 0.25& 1& 2.70& & \ldots& \ldots& 41.71 & -1.95 & \ldots & early\\

